Unitless Frobenius quantales

It is often stated that Frobenius quantales are necessarily unital. By taking negation as a primitive operation, we can define Frobenius quantales that may not have a unit. We develop the elementary theory of these structures and show, in particular, how to define nuclei whose quotients are Frobenius quantales. This yields a phase semantics and a representation theorem via phase quantales. Important examples of these structures arise from Raney's notion of tight Galois connection: tight endomaps of a complete lattice always form a Girard quantale which is unital if and only if the lattice is completely distributive. We give a characterisation and an enumeration of tight endomaps of the diamond lattices Mn and exemplify the Frobenius structure on these maps. By means of phase semantics, we exhibit analogous examples built up from trace class operators on an infinite dimensional Hilbert space. Finally, we argue that units cannot be properly added to Frobenius quantales: every possible extention to a unital quantale fails to preserve negations.

==> macros.tex <==
\RequirePackage{hyperref}
\hypersetup{
  colorlinks=true,
  citecolor=blue,
  linkcolor=blue,
}




\RequirePackage{amsmath,amsthm,amssymb,amsfonts}
\RequirePackage{xspace}
\RequirePackage{xcolor}
\RequirePackage{graphicx}
\graphicspath{{figs/},{./}}
\DeclareGraphicsExtensions{.pdf}

\ifacs
\renewcommand{\S}{\textsection}
\fi

\ifacs
\renewcommand{\END}{\end{document}}
\else
\newcommand{\END}{\end{document}}
\fi




\newtheorem{proposition}{Proposition}
\newtheorem{definition}[proposition]{Definition}
\newtheorem{lemma}[proposition]{Lemma}
\newtheorem{theorem}[proposition]{Theorem}
\newtheorem{corollary}[proposition]{Corollary}

\theoremstyle{remark}
\newtheorem{remark}{Remark}
\newtheorem{notation}{Notation}
\newtheorem{conjecture}{Conjecture}

\newtheoremstyle{exmpl}
{3pt}
{3pt}
{}
{}
{\bf}
{.}
{.5em}
{\thmname{#1}\thmnumber{ #2}\thmnote{: {\bf #3}}}

\theoremstyle{exmpl}
\newtheorem{example}[proposition]{Example}
\newcommand{\qedExample}{\hfill$\Diamond$}
\RequirePackage{ifthen}
\newenvironment{Example}[1][]{\bigskip\ifthenelse{\equal{#1}{}}{\begin{example}}{\begin{example}[#1]}}{\qedExample\end{example}}

\newcommand{\Myparagraph}[1]{\bigskip\paragraph{\bf #1}}



\newcommand{\trup}[1]{{#1}^{\sharp}}
\newcommand{\Trup}[1]{\trup{(#1)}}
\newcommand{\tr}[1]{\trup{#1}}
\newcommand{\trdown}[1]{{#1}^{\flat}}
\newcommand{\Trdown}[1]{\trdown{(#1)}}
\newcommand{\FUN}{(\,-\,)}
\newcommand{\trupMap}{\trup{\FUN}}
\newcommand{\trdownMap}{\trdown{\FUN}}


\newcommand{\IHom}[1]{[#1]}
\newcommand{\Hom}[1]{\hom(#1)}
\newcommand{\Star}[1]{{#1}^{\ast}}
\newcommand{\STAR}[1]{#1{}^{\ast}}
\newcommand{\SStar}[1]{{#1}\Star{}\Star{}}
\newcommand{\SSStar}[1]{\SStar{#1}{}^{\ast}}
\newcommand{\Perp}[1]{{#1}^{\perp}}
\renewcommand{\Tilde}[1]{\widetilde{#1}}


\newcommand{\HSS}{\IHom{S,S}}

\newcommand{\SI}{\Star{I}}
\newcommand{\SSI}{\SStar{I}}
\newcommand{\SX}{\Star{X}}
\newcommand{\SY}{\Star{Y}}
\newcommand{\SSX}{\SStar{X}}
\newcommand{\SSY}{\SStar{Y}}
\newcommand{\SSSX}{\SSStar{X}}
\newcommand{\SSSY}{\SSStar{Y}}
\newcommand{\HXY}{\IHom{X,Y}}
\newcommand{\HYX}{\IHom{Y,X}}
\newcommand{\HSYSX}{\IHom{\SY,\SX}}
\newcommand{\SM}{\Star{M}}
\newcommand{\SSM}{\Star{M}\Star{}}
\newcommand{\SQ}{\Star{Q}}
\newcommand{\SSQ}{\Star{Q}\Star{}}
\newcommand{\SA}{\Star{A}}
\newcommand{\SSA}{\SStar{A}}
\renewcommand{\SS}{\Star{S}}
\newcommand{\SSS}{\Star{S}\Star{}}
\newcommand{\SB}{\Star{B}}
\newcommand{\SC}{\Star{C}}

\newcommand{\HMM}{\IHom{M,M}}
\newcommand{\HSMSM}{\IHom{\SM,\SM}}

\newcommand{\ev}{ev}
\newcommand{\trace}{tr}

\newcommand{\rto}[1][\qquad]{\xrightarrow{#1}}
\newcommand{\Rto}[1][\qquad]{\xrightarrow{\;\;#1\;\;}}

\newcommand{\eqdef}{:=}
\newcommand{\smallLHS}[2][20mm]{\makebox[#1][l]{${\displaystyle #2}$}}


\newcommand{\tor}{\text{or}}
\newcommand{\Tor}{\;\;\tor\;\;}
\newcommand{\tand}{\text{and}}
\newcommand{\Tand}{\;\;\tand\;\;}
\newcommand{\tiff}{\text{iff}}
\newcommand{\Tiff}{\;\;\tiff\;\;}
\newcommand{\Timplies}{\;\;\text{implies}\;\;}
\newcommand{\Tst}{\;\;\tst\;\;}
\newcommand{\tst}{\text{s.t.}}


\ifacs
\renewcommand{\C}{\mathbb{C}}
\else
\newcommand{\C}{\mathbb{C}}
\fi

\newcommand{\homm}[2]{[#1, #2]} 
\newcommand{\ri}{\operatorname{r}}
\newcommand{\li}{\operatorname{l}}




\newcommand{\tensor}{\otimes}
\newcommand{\tesnor}{\otimes}
\newcommand{\cotensor}{\oplus}
\newcommand{\parr}{\rotatebox[origin=c]{180}{$\mathcal{\&}$}}
\newcommand{\comult}{\parr}



\newcommand{\bil}[1][\cdot]{\langle#1\rangle}
\renewcommand{\brack}[1]{\bil[#1]}
\newcommand{\bilr}[1][\cdot]{\bil[#1]{}^{\perp}}
\newcommand{\bill}[1][\cdot]{{}^{\perp}\bil[#1]}


\newcommand{\SLatt}{\ensuremath{\mathsf{SLatt}}\xspace}
\newcommand{\lrimpl}{\backslash}
\newcommand{\rlimpl}{/}
\newcommand{\rneg}[1][(\,\cdot\,)]{{#1}^{\perp}}
\newcommand{\lneg}[1][(\,\cdot\,)]{{}^{\perp}{#1}}
\newcommand{\Rneg}[1]{{#1}{}^{\perp}}
\newcommand{\Dneg}[1]{\Rneg{#1}\Rneg{}}
\newcommand{\Lneg}[1]{{}^{\perp}{#1}}
\newcommand{\Loplus}{\,{}_{\perp}\!\!\oplus}
\newcommand{\Roplus}{\oplus_{\perp}}

\newcommand{\SLTL}{\SL\tensor L}
\newcommand{\LTSL}{L\tensor \SL}
\newcommand{\SLtL}{\SLTL}
\newcommand{\HLL}{\IHom{L,L}}
\newcommand{\HSLSL}{\IHom{\SL,\SL}}


\newcommand{\myqedhere}[1][0mm]{
  \mbox{
    \begin{tabular}[t]{@{\hspace{0mm}}r@{\hspace{0mm}}}
      \\[#1]
      \qedhere
    \end{tabular}
  }
}

\newcommand{\Fsg}{Frobenius semigroup\xspace}
\newcommand{\iso}{\simeq}
\newcommand{\V}{\ensuremath{\mathcal{V}}}

\newcommand{\Rans}[1]{{#1}^{\vee}}
\newcommand{\Rani}[1]{{#1}^{\wedge}}
\newcommand{\rans}[1]{{#1}{}^{\vee}}
\newcommand{\rani}[1]{{#1}{}^{\wedge}}

\newcommand{\rand}[1]{#1\rani{}\rans{}}
\newcommand{\ranD}[1]{#1\rans{}\rani{}}
\newcommand{\Homs}[1]{{\homm{#1}{#1}}_{\vee}}
\newcommand{\LLs}{{\homm{L}{L}}_{\vee}}
\newcommand{\LLi}{{\homm{L}{L}}_{\wedge}}
\newcommand{\LLst}{\LLs^{t}}
\newcommand{\LLit}{\LLi^{t}}
\newcommand{\LLt}{\LLst}

\newcommand{\mix}{\mathtt{mix}}
\newcommand{\SL}{\Star{L}}
\newcommand{\SSL}{\SStar{L}}
\newcommand{\op}{\operatorname{op}}
\newcommand{\Ld}{{L}^{\op}}
\newcommand{\Md}{{M}^{\op}}
\newcommand{\Qd}{{Q}^{\op}}
\newcommand{\SYTX}{\Star{(\SY\tensor X)}}


\newcommand{\ifff}{\text{  iff  }}
\newcommand{\Ifff}{\quad\text{iff}\quad}
\newcommand{\st}{\text{  s.t.  }}
\newcommand{\contr}{a contradiction\xspace}
\newcommand{\Impl}[2]{(#1) $\Rightarrow$ (#2)}
\newcommand{\ra}{right-adjoint\xspace}
\newcommand{\la}{left-adjoint\xspace}
\newcommand{\jp}{sup-preserving\xspace}
\renewcommand{\mp}{inf-preserving\xspace}
\newcommand{\LL}{L^{L}}

\newcommand{\fun}{(-)}
\newcommand{\adj}{\dashv}
\newcommand{\rightIso}[1]{\xrightarrow{\,\overset{\raisebox{4pt}{{$\scriptsize
          #1$}}}{\raisebox{-4pt}{$\tiny \sim$}}\,}}
\newcommand{\rIso}[1]{\rightIso{#1}}

\newcommand{\bm}{bracketed magma\xspace}
\newcommand{\id}{\mathtt{id}}

\newcommand{\lact}[1][A]{\alpha^{\ell}_{#1}}
\newcommand{\ract}[1][B]{\alpha^{\rho}_{#1}}
\newcommand{\affine}{affine\xspace}

\newcounter{useDiagCount}
\setcounter{useDiagCount}{0}
\newcommand{\useDiagram}[2][]{
  \ifthenelse{\isinteger{#1}}{
    \setcounter{useDiagCount}{#1}
    \includegraphics[page=#1,align=c]{#2}
  }{
    \stepcounter{useDiagCount}
    \def\page{\theuseDiagCount}
    \includegraphics[page=\page,align=c,#1]{#2}
  }
}

\newcommand{\cl}{complete lattice\xspace}
\newcommand{\cd}{completely distributive\xspace}
\newcommand{\cdlatt}{\cd lattice\xspace}
\newcommand{\upTensor}{\widehat{\tensor}}
\newcommand{\RT}{Raney's theorem\xspace}

\ifacs
\renewcommand{\set}[1]{\{ \,#1\,\}}
\else
\newcommand{\set}[1]{\{ \,#1\,\}}
\fi
\newcommand{\downset}[1]{\downarrow #1}
\newcommand{\two}{\mathbf{2}}
\newcommand{\closure}[1]{\overline{#1}}
\newcommand{\positive}{positive\xspace}
\newcommand{\strong}{strongly continuous\xspace}

\newcommand{\card}[1]{\lvert #1\rvert}

\newcommand{\leftA}{l}
\newcommand{\rightA}{r}
\newcommand{\leftB}{\lambda}
\newcommand{\rightB}{\rho}
\newcommand{\F}{\mathbb{F}}
\newcommand{\K}{\mathbb{K}}
\newcommand{\pairing}[1]{\langle#1\rangle}
\newcommand{\Pairing}[1]{(#1)}
\newcommand{\innerH}[1]{\pairing{#1}_{H}}
\newcommand{\normH}[1]{||#1||_{H}}

\newcommand{\qmult}{\ast}
\newcommand{\Cstar}{\ensuremath{\mathrm{C}^{\ast}}}

\newcommand{\saut}{$\ast$-autonomous\xspace}
\newcommand{\sautcat}{\saut category\xspace}
\newcommand{\sautcats}{\saut categories\xspace}
\newcommand{\autcat}{autonomous category\xspace}
\newcommand{\autcats}{autonomous categories\xspace}

\newcommand{\radj}[1]{\rho(#1)}
\newcommand{\ladj}[1]{\ell(#1)}
\newcommand{\supj}{\mbox{$\bigvee_j$}}
\newcommand{\cotight}{cotight\xspace}


